Querying Linked Data: how to ensure user's quality requirements

In the distributed and dynamic framework of the Web, data quality is a big challenge. The Linked Open Data (LOD) provides an enormous amount of data, the quality of which is difficult to control. Quality is intrinsically a matter of usage, so consumers need ways to specify quality rules that make sense for their use, in order to get only data conforming to these rules. We propose a user-side query framework equipped with a checker of constraints and confidence levels on data resulting from LOD providers\' query evaluations. We detail its theoretical foundations and we provide experimental results showing that the check additional cost is reasonable and that integrating the constraints in the queries further improves it significantly.

==> comp-NaiveAlgo.tex <==
%%% NAIVE APPROACH


The main idea of the naive approach is to validate each answer of a query $q$ by generating sub-queries corresponding to each constraint $c \in \C$. 
The process consists of three steps: (i) evaluate   $q$ to obtain a set of candidate answers $\R'$, 
(ii) generate  sub-queries from each answer in $\R'$, for each constraint $c \in \C$, and 
(iii) evaluate the sub-queries and decide the validity of the answer.
The final set $\R$ contain only valid answers.


 Let $h_t$ be the homomorphism used to produce tuple $t \in \R'$ as an answer for $q$.
%Given a query $q$, let $h_t$ be the homomorphism used to produce tuple $t \in \R'$ as an answer for $q$.
%We want to check whether $t$ is valid \wrt\ constraints.
Tuple $t$ is a \textit{valid answer} only when \textit{all} constraints triggered during the validation process are satisfied.
The instantiation $h_t (L(\X))$ (of an atom $L(\X)$ in  $body(q)$) may trigger constraint $c$.
%Let $L(\X)$ be an atom of $ body(q)$.
%The instantiated atom $h_t (L(\X))$ may trigger a constraint $c$.
According to  the type of  %the triggered constraint 
$c$,  a suitable sub-query $q'$ is created:

%\begin{itemize}\item %
\noindent
$(i)$  	For $c \in \C_P$, $q'$ is a boolean query: $q'() \leftarrow  h_t(L_0(\X_0))$ where
	$ L_0(\X_0) =head(c)$. The resulting tuple $t$ is valid \wrt\  $c$  if the answer of $q'$  is positive. 
	Each fact $f$ resulting from the instantiation  of $h_t(L_0(\X_0))$  in the database may trigger another constraint. 
	The validation process continues until no constraint is triggered as stated by the use of $h_1$ in Definition~\ref{def:ValAns}, which corresponds to a chase procedure. This process establishes a dialogue between the validator and the providers.\\
% This is done in Algorithm~\ref{algo:naive} by the recursive call in line~\ref{algoNaive:recursive}.
%	\item %
$(ii)$  For $c \in \C_N$ and assuming that $c$ has the form $L(\X), L_0(\X_0) \rightarrow \bot$ the \ignore{auxiliary} boolean sub-query is $q'() \leftarrow h_t (L_0(\X_0)).$  Tuple $t$ is valid \wrt\  $c$ if the answer of $q'$ is negative. %(line~\ref{algo:naive_CN2}).
	Clearly,  if $c$ has the form $L(\X) \rightarrow \bot$,  the verification is straightforward. \\
	%(line~\ref{algo:naive_CN1}).
%	\item %
$(iii)$ 
	For $c \in \C_K$,   assuming that $c$ has form $L(\Y, X_1, \Z_1), L_0(\Y, $ $X_2,\Z_2) \rightarrow X_1 = X_2$  and $\X = \Y \cup X_1 \cup \Z_1$,
	the \ignore{auxiliary} sub-query is 
	$q'(X_2) \leftarrow  h_t(L_0(\Y, X_2,$ $\Z_2)) $.
	Tuple $t$ is valid \wrt\ $c$ if the answer set 
	is a singleton containing the tuple value $h_t(X_1)$.  %(line~\ref{algo:naive_Ck}).
%\end{itemize}




